Cormorant: Covariant Molecular Neural Networks

We propose Cormorant, a rotationally covariant neural network architecture for learning the behavior and properties of complex many-body physical systems. We apply these networks to molecular systems with two goals: learning atomic potential energy surfaces for use in Molecular Dynamics simulations, and learning ground state properties of molecules calculated by Density Functional Theory. Some of the key features of our network are that (a) each neuron explicitly corresponds to a subset of atoms; (b) the activation of each neuron is covariant to rotations, ensuring that overall the network is fully rotationally invariant. Furthermore, the non-linearity in our network is based upon tensor products and the Clebsch-Gordan decomposition, allowing the network to operate entirely in Fourier space. Cormorant significantly outperforms competing algorithms in learning molecular Potential Energy Surfaces from conformational geometries in the MD-17 dataset, and is competitive with other methods at learning geometric, energetic, electronic, and thermodynamic properties of molecules on the GDB-9 dataset.

==> supplement_cglayers.tex <==
\section{Covariant $\SO(3)$-vector layers}
\label{sec:cg_layers}

We discuss the specific implementation of the covariant CG layers acting on the $\SO(3)$-vector 
activations $F_i$. Our network is inspired by the $n \leq 3$-atom interactions described in the main text. 
In practice, computational limitations forced us to take only a subset of these operations, in particular:  
%The set of operations we include in our CG-layer is:
\begin{equation}
%\mathrm{CGLayer}(\{F_{i},\mathbf{r}_{ij}\})=
\bigg[
\underbrace{\Big(F_{i}\oplus\brBig{\sum_{j}\Upsilon_{ij}^{\left(1\right)}\otimescg F_{j}}\Big)}_{\textrm{one-body}}
\oplus\underbrace{\left(F_{i}\otimescg F_{i}\right)}_{\textrm{two-body}}
%\oplus\underbrace{\left(F_{i}\right)^{\otimescg 2}}_{\textrm{two-body}}
%\oplus\underbrace{\left(\sum_{j}F_{i}\otimescg\Upsilon_{ij}^{\left(3\right)}\otimescg F_{j}\otimescg F_{j}\right)}_{\textrm{three-body}}
\oplus\underbrace{\Big(\sum_{j}F_{i}\otimescg\Upsilon_{ij}^{\left(3\right)}\otimescg \left(F_{j}\right)^{\otimescg 2}\Big)}_{\textrm{three-body}}
\bigg] \cdot W
\end{equation}
%
%\begin{align*}
%\mathrm{CGLayer}(\{F_{i},\mathbf{r}_{ij}\})&=F_{i}\oplus(\sum_{j}\Upsilon_{ij}\otimescg F_{j})\oplus\left(F_{i}\otimescg F_{i}\right)\oplus\big((\sum_{j}F_{i}\otimescg\Upsilon_{ij}\otimescg F_{j})\otimescg F_{j}\big)\\&=\sum_{j}\left(\delta_{ij}\oplus\Upsilon_{ij}\oplus\delta_{ij}F_{i}\oplus\big(F_{i}\otimescg\Upsilon_{ij}\otimescg F_{j}\big)\right)\otimescg F_{j}
%\end{align*}
For computational tractability, we replace 
$F_{i}\otimescg\Upsilon_{ij}^{\left(3\right)}\otimescg F_{j}$ by $(F_{i}\cdot F_{j}) \otimescg\Upsilon_{ij}^{\left(3\right)}$ in the three-body term. This can be be done 
using the properties of the CG transformation to give a unitary redefinition of $W \rightarrow W^\prime$, 
followed by a projection into the subspace for which $\ell_{\rm max} = 0$. 
After some algebra, we arrive at the form of our $\mathrm{CGLayer}$:
\begin{equation}
\mathrm{CGLayer}(\{F_{i},\mathbf{r}_{ij}\}) = 
\Big[F_i \oplus 
\big( F_{i}\otimescg F_{i}\big) \oplus 
\Big(\sum_{j}\Big(\Upsilon_{ij}^{\left(1\right)}\oplus 
\big(F_{i}\cdot F_{j}\big) \Upsilon_{ij}^{\left(3\right)}\Big)\otimescg F_{j} \big)\Big] 
\cdot W^\prime
\label{eq:cglayer-mpnn}
\end{equation}
%This is the basic structure of the $\mathrm{CGLayer}$-s we use in our networks. 

%\subsubsection{Edge networks}
%\label{sec:edge_networks}

Structurally, \rf{eq:cglayer-mpnn} looks similar to a message passing neural network 
\citep{Gilmer2017}), where messages are CG-products acting on $\SO(3)$-vector activations. 
%$\mathcal{E}^{s}_{ij} = $
In this framework, the term 
\sm{\Upsilon_{ij}^{\left(\mathrm{edge}\right)}  = \Upsilon_{ij}^{\left(1\right)}\oplus\left(F_{i}\cdot F_{j}\right)\Upsilon_{ij}^{\left(3\right)}} 
looks like an ``edge network'' with $\SO(3)$-vector messages. %~(\cite{Riley2017}). 
Inspired by this connection, we generalize our architecture to 
\begin{equation}
%\mathrm{CGLayer}(\{F_{i},\mathbf{r}_{ij}\}) = 
%\Big[\sum_{j}\left(\delta_{ij}\oplus\delta_{ij}F_{i}\oplus \mathcal{E}^{s}_{ij}\right)\otimescg F_{j}\Big] \cdot W^\prime 
\mathrm{CGLayer}(\{F_{i},\mathbf{r}_{ij}\}) = 
\Big[
F_i \oplus \big( F_{i}\otimescg F_{i}\big) \oplus 
\big( \sum_{j} \Upsilon_{ij}^{\left(\mathrm{edge}\right),s} \otimescg F_{j} \big)\Big] \cdot W^\prime.
\label{eq:cglayer-edge}
\end{equation}
Following this idea, we can allow the edge network to be ``self-consistently'' updated based upon the value at the previous level: 
\m{\Upsilon_{ij}^{\left(\mathrm{edge}\right),s} \equiv \big[ \Upsilon_{ij}^{\left(\mathrm{edge}\right),s-1} \oplus \Upsilon_{ij}^{\left(1\right),s}\oplus\big(F_{i}\cdot F_{j}\big)\Upsilon_{ij}^{\left(3\right),s} \big] \cdot W_{\mathrm{edge}}} is a ``self-consistent'' amplitude.
In practice, we assume $\Upsilon_{ij}^{\left(1,3\right),s} \propto Y^\ell(\hat{\mathbf{r}}_{ij})$. We can therefore calculate the edge network by defining $\Upsilon_{ij}^{\left(\mathrm{edge}\right),s}  = \bigoplus_{\ell=0}^{\ell_{\rm max}} \mathcal{E}^{s,\ell}_{ij} Y^\ell(\hat{\mathbf{r}}_{ij})$, and then updating 
\sm{\mathcal{E}^{s}_{ij} = \bigl( \mathcal{E}^{s-1}_{ij} \oplus \mathcal{F}^{(1),s}_{ij} \oplus \mathcal{D}^{s}_{ij} \bigr) \cdot W_{\rm edge}}, 
where $\mathcal{D}^{s}_{ij} = (F_{i}\cdot F_{j})$. 

%This replacement results in a $\mathrm{CGLayer}$ architecture defined by

%where 

%is an edge network that accounts for both one-body aggregation and a limited form of three-body interactions.

%\subsubsection{Masks and local environments}
%\label{sec:marks_local}

The functions $\Upsilon_{ij}$ define the position dependence of the interaction between atoms $i$ and $j$. In chemical environments, atoms that are separated by a significant distance will not talk to each other. For this reason we include a soft mask $\Upsilon_{ij} \rightarrow m_{ij} \times \Upsilon_{ij}$, where $m_{ij} = \sigma((r_{\rm cut} - r_{ij}) / w)$, and $r_{\rm cut}$, $w$ are respectively learnable cutoffs and widths described below.



==> supplement_interactions.tex <==
\section{General $n$-atom Interaction terms}

We now write the general form of the $n$-atom interactions described in the main text. 

\begin{equation}

\end{equation}

==> table_symbols.tex <==
\begin{table}[tb]
\begin{tabular}{|c|l|}
\hline 
Symbol & Meaning\tabularnewline
\hline 
\hline 
$Z_{i}$ & Atomic charge of atom $i$ (e.g., Hydrogen would be $Z_{i}=1$, and
Carbon would be $Z_{i}=6$)\tabularnewline
\hline 
$\mathbf{r}_{i}$ & Position of atom $i$\tabularnewline
\hline 
$\mathbf{r}_{ij}$ & Relative position of atoms $i$ and $j$: $\mathbf{r}_{ij}=\mathbf{r}_{i}-\mathbf{r}_{j}$\tabularnewline
\hline 
$\hat{\mathbf{r}}_{ij}$ & Unit vector in the direction of $\mathbf{r}_{ij}$\tabularnewline
\hline 
$s$ & Index of a ${\rm CGLayer}$ in Cormorant\tabularnewline
\hline 
$S$ & Top ${\rm CGLayer}$\tabularnewline
\hline 
$\ell$ & Index of an irreducible representation of ${\rm SO\left(3\right)}$\tabularnewline
\hline 
$L$ & Largest index in a representation\tabularnewline
\hline 
$m$ & Component $m\in[-\ell,\ell]$ of a ${\rm SO\left(3\right)}$-vector\tabularnewline
\hline 
$\tau^{s}$ & Vector of multiplicities of a ${\rm SO\left(3\right)}$-vector at
layer $s$\tabularnewline
\hline 
$n_{c}$ & Number of output channels of a ${\rm CGLayer}$\tabularnewline
\hline 
$\bar{V}_{\ell}$ & Representation space for irrep with index $\ell$ and multiplicity
$\tau_{\ell}=1$: $\bar{V}_{\ell}=\mathbb{C}^{\left(2\ell+1\right)\times1}$\tabularnewline
\hline 
$V^{s}$ & Representation space for ${\rm SO\left(3\right)}$-vector of type
$\tau^{s}$: $V^{s}=\bigoplus_{\ell=0}^{L}\bar{V}_{\ell}^{\tau_{\ell}^{s}}$\tabularnewline
\hline 
$V_{{\rm edge}}^{s}$ & Vector space for an scalar edge network at layer $s$: $V_{{\rm edge}}^{s}=\bigoplus_{\ell=0}^{L}\mathbb{C}^{\tau_{\ell}^{s}}$\tabularnewline
\hline 
$F_{i}^{s}$ & ${\rm SO\left(3\right)}$-vector atom-activation at layer $s$ for
atom $i$ \tabularnewline
\hline 
$Y^{\ell}\left(\hat{\mathbf{r}}_{ij}\right)$ & Spherical harmonics of weight $\ell$ in the direction of $\hat{\mathbf{r}}_{ij}$\tabularnewline
\hline 
$Y_{ij}$ & ${\rm SO\left(3\right)}$-vector of spherical harmonics connecting
atoms $i$ and $j$: $Y_{ij}=\bigoplus_{\ell=0}^{L}Y^{\ell}\left(\hat{\mathbf{r}}_{ij}\right)$\tabularnewline
\hline 
$g_{ij}^{s}$ & Scalar edge activation layer $s$ connecting atoms $i$ and $j$\tabularnewline
\hline 
$d_{ij}^{s}$ & Scalar matrix of dot products $d_{ij}^{s}=F_{i}^{s}\cdot F_{j}^{s}$\tabularnewline
\hline 
$\eta_{ij}^{s}$ & Radial basis functions between atoms $i$ and $j$\tabularnewline
\hline 
$G_{ij}^{s}$ & ${\rm SO\left(3\right)}$-vector edge activation layer $s$ connecting
atoms $i$ and $j$\tabularnewline
\hline 
$W_{s,\ell}^{{\rm vertex}}$ & Weight mixing matrix for component $\ell$ of atom ${\rm SO\left(3\right)}$-vector
activations at layer $s$\tabularnewline
\hline 
$W_{s,\ell}^{{\rm edge}}$ & Weight mixing matrix for component $\ell$ of scalar edge activations
at layer $s$\tabularnewline
\hline 
\end{tabular}

\caption{\label{tab:symbols}Table of symbols used in the main text and supplement.}
\end{table}
